Beyond Average Hamiltonian Theory for Quantum Sensing

The application of average Hamiltonian theory (AHT) to magnetic resonance and quantum sensing informs pulse sequence design, for example, by providing efficient approximations of spin dynamics while retaining important physical characteristics of system evolution. However, AHT predictions break down in many common experimental conditions, including for sensing with solid-state spins. Here we establish that certain symmetries, such as rapid echos, allow AHT to remain accurate well beyond the perturbative limit. An exact method is presented to determine the sensor response to a target signal, which stays valid beyond the regime of AHT convergence. This beyond AHT approach enables new opportunities in quantum control techniques that leverage complementary analytical and numerical methods, with applications in a variety of quantum sensing platforms, Hamiltonian engineering, and probes of quantum many-body phenomena.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

